BaDExpert: Extracting Backdoor Functionality for Accurate Backdoor Input Detection

We present a novel defense, against backdoor attacks on Deep Neural Networks (DNNs), wherein adversaries covertly implant malicious behaviors (backdoors) into DNNs. Our defense falls within the category of post-development defenses that operate independently of how the model was generated. The proposed defense is built upon a novel reverse engineering approach that can directly extract backdoor functionality of a given backdoored model to a backdoor expert model. The approach is straightforward -- finetuning the backdoored model over a small set of intentionally mislabeled clean samples, such that it unlearns the normal functionality while still preserving the backdoor functionality, and thus resulting in a model (dubbed a backdoor expert model) that can only recognize backdoor inputs. Based on the extracted backdoor expert model, we show the feasibility of devising highly accurate backdoor input detectors that filter out the backdoor inputs during model inference. Further augmented by an ensemble strategy with a finetuned auxiliary model, our defense, BaDExpert (Backdoor Input Detection with Backdoor Expert), effectively mitigates 17 SOTA backdoor attacks while minimally impacting clean utility. The effectiveness of BaDExpert has been verified on multiple datasets (CIFAR10, GTSRB and ImageNet) across various model architectures (ResNet, VGG, MobileNetV2 and Vision Transformer).

==> assets/alg_detection_v0.tex <==
\begin{minipage}{0.48\textwidth}

\begin{algorithm}[H]
\caption{Backdoor Input Detection with Backdoor Experts (Ver 0)}

\textbf{Input:} Input $x$, Model $\mathcal M$, Backdoor Expert $\mathcal B$\\
\textbf{Output:} Whether or not $x$ has triggered the potential backdoor within $\mathcal M$

\begin{algorithmic}[1]

  \State $\text{Pred}_\mathcal{M} \gets \arg\max_{i\in \mathcal [C]} \mathcal M_i(x)$
  \State $\text{Pred}_\mathcal{B} \gets \arg\max_{i\in \mathcal [C]} \mathcal B_i(x)$
  
  \State \Return ($\text{Pred}_\mathcal{M} = \text{Pred}_\mathcal{B}$)

\end{algorithmic}

\label{alg:alg-detection-v0}
\end{algorithm}



\begin{algorithm}[H]
\caption{Backdoor Input Detection with Backdoor Experts (Ver 1)}

\textbf{Input:} Input $x$, Model $\mathcal M$, Backdoor Expert $\mathcal B$, Finetuned Model $\mathcal M'$\\ %Small Clean Dataset $D_c$\\
\textbf{Output:} Whether or not $x$ has triggered the potential backdoor within $\mathcal M$

\begin{algorithmic}[1]

  % \State $\mathcal{M'} \gets$ Finetuning $\mathcal M$ on $D_c$
  \State $\Tilde{y} \gets \arg\max_{i\in \mathcal [C]} \mathcal M_i(x)$
  \State $\text{Conf}_\mathcal{B} \gets \mathcal B_{\text{Pred}_\mathcal{M}}(x)$
  \State $\text{Conf}_\mathcal{M'} \gets \mathcal M'_{\text{Pred}_\mathcal{M}}(x)$
  \State \Return

\end{algorithmic}

\label{alg:alg-detection-v1}
\end{algorithm}



\end{minipage}

==> assets/alg_detection_v1.tex <==
\begin{minipage}{0.48\textwidth}

\begin{algorithm}[H]
\caption{Backdoor Samples Detection with Backdoor Experts (Ver 1)}

\textbf{Input:} Input $x$, Model $\mathcal M$, Backdoor Expert $\mathcal B$\\
\textbf{Output:} Whether or not $x$ has triggered the potential backdoor within $\mathcal M$

\begin{algorithmic}[1]

  \State $\text{Pred}_\mathcal{M} \gets \arg\max_i \mathcal M(x)$
  \State $\text{Pred}_\mathcal{B} \gets \arg\max_i \mathcal B(x)$
  
  \State \Return ($\text{Pred}_\mathcal{M} == \text{Pred}_\mathcal{B}$)

% \For{$i=1,...,m$}\Comment{Confusion Training}
%       \State $(\mathbf{\widetilde{X}}_i, \mathbf{\widetilde{Y}}_i) \gets$ a random batch from $Dpoiall$  \label{line:poison-batch}                 
%       \State $({\mathbf X}'_i, {\mathbf Y}'_i) \gets$ a random batch from $D$ \label{line:clean-batch}         
%       \State ${\mathbf Y}^* \gets$ random mislabels other than ${\mathbf Y}'_i$  \label{line:random-mislabel}  
%       \State $\ell_{ct} \gets  \frac{loss(f(\mathbf{\widetilde{X}}_i;\theta_{ct}), \mathbf{\widetilde{Y}}_i) + (\lambda-1) \cdot  loss(f({\mathbf X}'_i;\theta_{ct}), \mathbf{Y}^*)}{\lambda}$ \label{line:confusion-loss}  
%       \State $D \gets$ one step gradient descent on $\ell_{\text{ct}}$
% \EndFor\label{line:end_of_confusion_training}

% \State $D^* \gets Dpoiall$

% \For{$i=1,...,n$} \label{line:start-of-detection} \Comment{Poison Detection}
% \If{$\Tilde{y}_i == F(\Tilde{x}_i;\theta_{ct})$} \label{line:decision-rule}
% \State $D^* \gets$ remove $(\Tilde{x}_i, \Tilde{y}_i)$ from $D^*$
% \EndIf
% \EndFor \label{line:end-of-detection}
% \State \Return $D^*$

\end{algorithmic}

\label{alg:alg-detection-v1}
\end{algorithm}

\end{minipage}

==> assets/overview.tex <==
\begin{figure}[t]
% \vspace{-2em}
\begin{center}
\includegraphics[width=1\textwidth]{fig/overview.pdf}
\end{center}
\caption{
An overview of our BaDExpert pipeline to detect backdoor inputs with the backdoor expert. 
}
\label{fig:overview}
\end{figure}

==> assets/overview_backdoor_expert_only.tex <==
\begin{figure}[t]
\vspace{-2em}
\begin{center}
\includegraphics[width=1\textwidth]{fig/overview_backdoor_expert_only.pdf}
\end{center}
\caption{
\textbf{Utilizing backdoor experts for backdoor input detection.} The backdoor expert model $\B$ retains only backdoor functionality. As such, a backdoor input that successfully deceives $\M$ (predicted to ``Dog'') will likewise obtain the same prediction (``Dog'') by $\B$ --- \underline{$\B$ \textbf{agrees} with $\M$}. Conversely, since $\B$ lacks the normal functionality, it cannot recognize the clean input as $\M$ does (correctly predict to ``Cat''), and will thus provide a possibly divergent prediction (e.g. ``Fish'') --- \underline{$\B$ \textbf{disagrees} with $\M$}. Based on the distinctive natures of clean and backdoor inputs, we can detect backdoor inputs at inference time by checking if $\B$ and $\M$ agree in predictions.
}
\label{fig:overview-backdoor-experts-only}
\vspace{-5mm}
\end{figure}


==> assets/suboptimal_unlearning_curves_demo.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.44\textwidth}
        \includegraphics[width=\textwidth]{fig/unlearning_curves/unlearning_curve_TrojanNN.png}
        \caption{Backdoor expert performance \small{(TrojanNN)}.}
        \label{fig:unlearning_curve-demo-TrojanNN}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.55\textwidth}
        \includegraphics[width=\textwidth]{fig/backdoor_experts_bar.png}
        \caption{Backdoor experts' performance (conservatively small $\eta$).}% across diverse attacks.}
        \label{fig:backdoor-experts-bar}
    \end{subfigure}
    \caption{Constructing optimal backdoor expert is difficult, ASR may also degrade when CA drops too much with a large $\eta$ (\ref{fig:unlearning_curve-demo-TrojanNN}). Rather, we extract backdoor functionality with a conservatively small $\eta$ (e.g. $10^{-4}$), where across all attacks, CA drops to only $\sim 30\%$ and ASR remains $\sim100\%$ (\ref{fig:backdoor-experts-bar}).}
    \label{fig:unlearning-curves-demo}
\end{figure}



==> tab/cifar_auroc.tex <==
\begin{table}[t]
\centering
\caption{\textbf{AUROC of BaDExpert and baseline backdoor input detectors. (CIFAR10)}}
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{lccccccccccccc}
\toprule
 \textbf{AUROC} ($\%$) & 
\multicolumn{1}{c}{BadNet} &
\multicolumn{1}{c}{Blend} &
\multicolumn{1}{c}{Trojan} &
\multicolumn{1}{c}{CL} &
\multicolumn{1}{c}{SIG} &
\multicolumn{1}{c}{Dynamic} &
\multicolumn{1}{c}{ISSBA} &
\multicolumn{1}{c}{WaNet} &
\multicolumn{1}{c}{Bpp} &
\multicolumn{1}{c}{FT} &
\multicolumn{1}{c}{TrojanNN} &
\multicolumn{1}{c}{SRA} &
\multicolumn{1}{c}{\textbf{Average}}\cr
\midrule

STRIP & 99.1 & 47.1 & 72.1 & 84.7 & 40.3 & 85.2 & 68.1 & 49.8 & 50.1 & 91.8 & 99.3 & 54.8 & 70.2 \cr
\midrule

AC & 100.0 & 54.1 & 99.7 & 99.9 & 53.6 & 77.9 & 84.4 & 47.2 & 98.4 & 58.7 & 99.9 & 99.6 & 81.1 \cr
\midrule

Frequency & 75.1 & 73.5 & 75.1 & 74.5 & 68.0 & 74.9 & 75.1 & 62.8 & 75.0 & 73.5 & 75.0 & 75.1 & 73.1 \cr
\midrule

SCALE-UP & 96.4 & 80.9 & 91.2 & 96.3 & 69.6 & 96.0 & 71.6 & 66.3 & 87.9 & 89.6 & 96.5 & 59.9 & 83.5 \cr
\midrule

\textbf{BaDExpert} & \textbf{100.0} & \textbf{99.0} & 99.2 & 99.0 & \textbf{99.8} & \textbf{99.1} & \textbf{96.1} & \textbf{99.7} & \textbf{100.0} & \textbf{99.6} & 99.3 & \textbf{100.0} & \textbf{99.0} \cr
\bottomrule

\end{tabular}
} % \resizebox
\label{tab:auroc_cifar10}
\end{table}


==> tab/wrap_generalizability_scalability_adaptive.tex <==
% \begin{wraptable}{r}{0.3\linewidth}

\begin{table}[t]
\vspace{-5mm}
\centering
\caption{BaDExpert generalizability on other architetures.}
\resizebox{0.3\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{lcc}
\toprule
 \textbf{AUROC} ($\%$) & 
\multicolumn{1}{c}{VGG16} &
\multicolumn{1}{c}{MobileNetV2} \cr
\midrule
BadNet & 99.7 & 99.5 \cr
\midrule
Blend & 97.7 & 97.6 \cr
\midrule
Trojan & 98.6 & 97.8 \cr
\midrule
CL & 97.7 & 99.2 \cr
\midrule
SIG & 98.4 & 98.9 \cr
\midrule
Dynamic & 96.7 & 98.1 \cr
\midrule
WaNet & 98.2 & 98.0 \cr
\midrule
FT & 99.3 & 98.7 \cr
\midrule
\textbf{Average} & \textbf{98.3} & \textbf{98.5} \cr
\bottomrule

\end{tabular}
} % \resizebox
\label{tab:ablation_arch_auroc}
% \end{table}
\vspace{-3mm}
% \end{wraptable}
% \begin{wraptable}{r}{0.6\linewidth}
% \begin{table}
% \vspace{-5mm}
\centering
% \caption{Adaptive attacks on BaDExpert.}
\resizebox{0.6\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{lccccc}
\toprule
 \textbf{AUROC} ($\%$) & 
\multicolumn{1}{c}{TaCT} &
\multicolumn{1}{c}{Adap-Blend} &
\multicolumn{1}{c}{Adap-Patch} &
\multicolumn{1}{c}{All-to-All} &
\multicolumn{1}{c}{\textbf{Average}}\cr
\midrule

STRIP & 44.8 & 61.9 & 95.4 & 8.7 & 52.7 \cr
\midrule

AC & 50.6 & 43.7 & 98.2 & 28.3 & 55.2 \cr
\midrule

Frequency & 74.9 & 73.7 & 75.2 & 75.0 & 74.7 \cr
\midrule

SCALE-UP & 61.3 & 79.4 & 96.2 & 48.6 & 71.4 \cr
\midrule

\textbf{BaDExpert} & \textbf{97.5} & \textbf{99.6} & \textbf{99.2} & \textbf{95.5} & \textbf{98.0} \cr
\bottomrule

\end{tabular}
} % \resizebox
\label{tab:adaptive_attacks}
\end{table}
% \end{wraptable}




\vspace{-5mm}
\begin{table}[H]
\centering
\caption{Defense results of BaDExpert on 1000-class ImageNet.}
\resizebox{0.75\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{llcccccccc}
\toprule
 & ($\%$) & 
% \multicolumn{4}{c}{ResNet} &
% \multicolumn{3}{c}{Vision Transformer} \cr
\multicolumn{3}{c}{ResNet18} &
\multicolumn{2}{c}{ResNet101} &
\multicolumn{3}{c}{ViT-B/16} \cr

\cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10}
% \cmidrule(lr){3-6} \cmidrule(lr){7-9}
 & &
\multicolumn{1}{c}{No Attack} &
\multicolumn{1}{c}{BadNet} &
\multicolumn{1}{c}{Blend} &
\multicolumn{1}{c}{No Attack} &
\multicolumn{1}{c}{SRA} &
\multicolumn{1}{c}{No Attack} &
\multicolumn{1}{c}{FT-BadNet} &
\multicolumn{1}{c}{FT-Blend} \cr

\multirow{2}*{\shortstack{Without Defense}}
& ACC & 69.0 & 68.4 & 69.0 & 77.1 & 74.7 & 81.9 & 82.3 & 81.8 \cr
& ASR & - & 100.0 & 92.2 & - & 100.0 & - & 99.5 & 93.2 \cr 
\midrule

\multirow{3}*{\shortstack{\textbf{BaDExpert}}}
& ACC & 68.9 & 68.3 & 68.9 & 77.0 & 74.6 & 81.8 & 82.2 & 81.7 \cr
& ASR & - & \grc 0.0 & \grc 4.9 & - & \grc 0.0 & - & \grc 0.0 & \grc 0.2 \cr
& AUROC & - &  100.0 & 99.9 & - & 100.0 & - & 100.0 & 100.0 \cr
\bottomrule

\end{tabular}
} % \resizebox
\label{tab:main_imagenet}
\end{table}
\vspace{-5mm}




